On Learning Closed-Loop Probabilistic Multi-Agent Simulator

The rapid iteration of autonomous vehicle (AV) deployments leads to increasing needs for building realistic and scalable multi-agent traffic simulators for efficient evaluation. Recent advances in this area focus on closed-loop simulators that enable generating diverse and interactive scenarios. This paper introduces Neural Interactive Agents (NIVA), a probabilistic framework for multi-agent simulation driven by a hierarchical Bayesian model that enables closed-loop, observation-conditioned simulation through autoregressive sampling from a latent, finite mixture of Gaussian distributions. We demonstrate how NIVA unifies preexisting sequence-to-sequence trajectory prediction models and emerging closed-loop simulation models trained on Next-token Prediction (NTP) from a Bayesian inference perspective. Experiments on the Waymo Open Motion Dataset demonstrate that NIVA attains competitive performance compared to the existing method while providing embellishing control over intentions and driving styles.

==> sections/2_related.tex <==
\section{Related Works}
\label{sec: related}

\subsection{Multi-agent Simulation for Autonomous Vehicles}
\label{subsec: review-av-simu}

Realistic and interactive simulation is critical to ensuring both the efficiency and safety of autonomous driving algorithms. Early studies in this field typically focused on improving open-loop fidelity based on recorded trajectories~\cite{Gao_2020_CVPR, NEURIPS2022_2ab47c96}. However, such methods did not account for the dynamic, interactive behaviors that appear in real-world traffic.

Recent benchmarks~\cite{NEURIPS2023_b96ce67b} have highlighted these shortcomings and spurred the development of closed-loop simulation frameworks. The primary difference lies in the modeling of conditional distributions: open-loop simulators predict future trajectories based solely on historical observations, while closed-loop simulators condition each action on the evolving history as the simulation unfolds. This new paradigm poses significant challenges in designing models that can efficiently sample and recursively refine generated trajectories. Early works in this area formulate traffic simulation as a Markov process and leverage recurrent models to capture dynamics~\cite{9561666, Suo_2021_CVPR}. More recently, inspired by the success of Large Language Models (LLMs)~\cite{brown2020languagemodelsfewshotlearners}, researchers have adopted Transformer architectures for autoregressive generation~\cite{vaswani2023attentionneed, zhang2024trafficbots, zhou2024behaviorgptsmartagentsimulation}, and some have even explored fine-tuning LLMs directly for scenario generation~\cite{pmlr-v229-zhong23a, 10629039}.

Despite these promising advances, a key challenge remains: Many existing models function as black boxes, offering limited interpretability of the learned behavioral dynamics and the underlying conditional structure. This opacity hinders the diagnosis of simulation errors, the refinement of generated scenarios, and adaptation to new conditions. Our work addresses this gap by training a probabilistic model that disentangles and explicitly parameterizes behavior styles, discrete intentions, and dynamics, providing robust simulation performance and enhanced interpretability.

\subsection{Probabilistic Generative Models in Simulation}
\label{subsec: review-gen-sim}

Probabilistic generative models have demonstrated invaluable capabilities for simulating complex, high-dimensional stochastic phenomena across various domains, ranging from weather forecasting~\cite{doi:10.1073/pnas.1810286115} to high-energy particle interactions~\cite{de2017learning}. Unlike deterministic simulators, probabilistic models explicitly learn the generative process underlying observations, thereby capturing inherent constraints and uncertainties as parameters or functions that encode richer information. Prior work has widely incorporated such probabilistic formulations: mixtures of Gaussian distributions are often employed to capture the multi-modality of human behavior~\cite{chai2019multipathmultipleprobabilisticanchor, NEURIPS2022_2ab47c96, 10398503}, while other studies have leveraged these models to enhance generalization~\cite{pmlr-v238-lu24a}, quantify uncertainty~\cite{Lu_2024_CVPR}, and improve controllability in scenario generation~\cite{10172005}.

However, despite their success in achieving high predictive accuracy and realism, the latent representations of many of these black-box models remain entangled. This entanglement results in limited controllability and interpretability of the learned dynamics and intentions. Motivated by these challenges, our work proposes a hierarchical Bayesian framework that explicitly disentangles continuous distributions representing behavior styles and dynamics from a discrete distribution capturing high-level intentions. Our method not only models the inherent stochasticity of traffic dynamics and human decisions but also provides interpretable latent representations that facilitate the generation of diverse and controllable simulation scenarios.
